Multi-BVOC Super-Resolution Exploiting Compounds Inter-Connection

Biogenic Volatile Organic Compounds (BVOCs) emitted from the terrestrial ecosystem into the Earth's atmosphere are an important component of atmospheric chemistry. Due to the scarcity of measurement, a reliable enhancement of BVOCs emission maps can aid in providing denser data for atmospheric chemical, climate, and air quality models. In this work, we propose a strategy to super-resolve coarse BVOC emission maps by simultaneously exploiting the contributions of different compounds. To this purpose, we first accurately investigate the spatial inter-connections between several BVOC species. Then, we exploit the found similarities to build a Multi-Image Super-Resolution (MISR) system, in which a number of emission maps associated with diverse compounds are aggregated to boost Super-Resolution (SR) performance. We compare different configurations regarding the species and the number of joined BVOCs. Our experimental results show that incorporating BVOCs' relationship into the process can substantially improve the accuracy of the super-resolved maps. Interestingly, the best results are achieved when we aggregate the emission maps of strongly uncorrelated compounds. This peculiarity seems to confirm what was already guessed for other data-domains, i.e., joined uncorrelated information are more helpful than correlated ones to boost MISR performance. Nonetheless, the proposed work represents the first attempt in SR of BVOC emissions through the fusion of multiple different compounds.

==> acronyms.tex <==
% Definitions
% --------------------
\newcommand{\HR}{\mathrm{\mathbf{I}_{HR}}}
\newcommand{\HRone}{\mathrm{\mathbf{I}_{HR_1}}}
\newcommand{\HRc}{\{\mathbf{I}_{\mathrm{HR}_c}\}}
\newcommand{\LR}{\mathrm{\mathbf{I}_{LR}}}
\newcommand{\LRc}{\mathbf{I}_{\mathrm{LR}_c}}
\newcommand{\HRt}{\mathrm{\mathbf{T}_{HR}}}
\newcommand{\THR}{\mathcal{T}(\mathrm{\mathbf{I}_{HR}})}
\newcommand{\THRhat}{\hat{\mathcal{T}}(\mathrm{\mathbf{I}_{HR}})}
\newcommand{\Tc}{\mathcal{T}_c}
\newcommand{\TLR}{\mathcal{T}(\mathrm{\mathbf{I}_{LR}})}
\newcommand{\TLRc}{\mathrm{\mathbf{T}_{\mathrm{LR}_c}}}
\newcommand{\LRt}{\mathrm{\mathbf{T}_{LR}}}
\newcommand{\HRhat}{\mathrm{\mathbf{\hat{I}}_{HR}}}
\newcommand{\HRhatone}{\mathrm{\mathbf{\hat{I}}_{HR_1}}}
\newcommand{\LRone}{\mathrm{\mathbf{I}_{LR_1}}}
\newcommand{\HRthat}{\mathrm{\hat{\mathbf{T}}_{HR}}}
\newcommand{\Net}{\mathcal{N}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\Tinv}{\mathcal{T}^{-1}}
\newcommand{\Tinvc}{\mathcal{T}_c^{-1}(\cdot)}
\newcommand{\Tq}{\mathcal{T}_\text{Q}}
\newcommand{\Ts}{\mathcal{T}_\text{S}}
\newcommand{\dcorr}{\mathcal{D}_{\text{con}}}
\newcommand{\duncorr}{\mathcal{D}_{\text{unc}}}
%\newcommand{\HRi}{\mathrm{\mathbf{I}_{HR_{1_i}}}}
\newcommand{\HRi}{\mathbf{I}_{\mathrm{HR}_{1_i}}}
\newcommand{\LRciset}{ \{\mathbf{I}_{\mathrm{LR}_{c}} \}_i}

% List of acronyms
% --------------------
\newacronym{voc}{VOC}{Volatile Organic Compound}
\newacronym{bvoc}{BVOC}{Biogenic Volatile Organic Compound}
\newacronym{sr}{SR}{Super-Resolution}
\newacronym{sisr}{SISR}{Single-Image Super-Resolution}
\newacronym{misr}{MISR}{Multi-Image Super-Resolution}
\newacronym{san}{SAN}{Second-order Attention Network}
\newacronym{nlrg}{NLRG}{Non-Locally Enhanced Residual Group}
\newacronym{lsrag}{LSRAG}{Local-Source Residual Attention Groups}
\newacronym{srgan}{SRGAN}{Super-Resolution Generative Adversarial Network}
\newacronym{esrgan}{ESRGAN}{Enhanced SRGAN}
\newacronym{srresnet}{SRResNet}{Super-Resolution ResNet}
\newacronym{msrresnet}{MSRResNet}{Modified SRResNet}
\newacronym{rcan}{RCAN}{Residual Channel Attention Network}
\newacronym{rrdbnet}{RRDBNet}{Residual-in-Residual Dense Block Network}
\newacronym{srcnn}{SRCNN}{Super-Resolution Convolutional Neural Network}
\newacronym{cdf}{CDF}{Cumulative Distribution Function}
\newacronym{hr}{HR}{High Resolution}
\newacronym{lr}{LR}{Low Resolution}
\newacronym{megan}{MEGAN}{Model of Emissions of Gases and Aerosols from Nature}
\newacronym{roc}{ROC}{Receiver Operating Characteristic}
\newacronym{auc}{AUC}{Area Under the Curve}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{nmse}{NMSE}{Normalized Mean Squared Error}
\newacronym{ssim}{SSIM}{Structural Similarity Index Measure}
\newacronym{pcc}{PCC}{Pearson Correlation Coefficient}
\newacronym{lst}{LST}{Land Surface Temperature}
\newacronym{sst}{SST}{Sea Surface Temperature}
\newacronym{vgg}{VGG}{Visual Geometry Group}
\newacronym{pinn}{PINN}{Physics-Informed Neural Networks}
\newacronym{stft}{STFT}{Short Time Fourier Transform}
\newacronym{dft}{DFT}{Discrete Fourier Transform}
\newacronym{dct}{DCT}{Discrete Cosine Transform}
\newacronym{cnn}{CNN}{Convolutional NN}
\newacronym{dl}{DL}{Deep Learning}
\newacronym{nn}{NN}{Neural Network}
\newacronym{mbsr}{MBSR}{Multi-BVOC Super-Resolution}
\newacronym{soa}{SOA}{Secondary Organic Aerosols}
\newacronym{ccn}{CCN}{Cloud Condensation Nuclei}
\newacronym{dwt}{DWT}{Discrete Wavelet Transforms}
\newacronym{ssw}{SSW}{Sea Surface Wind}
